Long-term monitoring of the radio-galaxy M87 in gamma-rays: joint analysis of MAGIC, VERITAS and Fermi-LAT data

M87 was discovered in the very-high-energy band (VHE, E > 100 GeV) with HEGRA in 2003, long before its emission was detected in the high-energy band (HE, E > 100 MeV) with Fermi-LAT in 2009, opening the window to a new family of extragalactic sources with tilted jets. After a series of major VHE flares in 2005, 2008, and 2010, which were detected in multiple bands, the source has been found in a low activity state, interrupted only by comparatively smaller-scale flares. MAGIC and VERITAS, two stereoscopic Cherenkov telescope arrays located at Roque de los Muchachos Observatory (Canary Islands, Spain) and the Fred Lawrence Whipple Observatory (Arizona, US), have monitored M87 continuously and in coordination for more than 10 years. In this work, we present the data for 4 years of MAGIC and VERITAS observations corresponding to 2019, 2020, 2021 and 2022. The resulting light curves are shown in daily and monthly scales where no significant variability is observed. In addition, we show the first joint analysis using combined event data from the two VHE instruments and Fermi-LAT to compute the spectral energy distribution.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

